Order Matters: Investigate the Position Bias in Multi-constraint Instruction Following

Real-world instructions with multiple constraints pose a significant challenge to existing large language models (LLMs). An observation is that the LLMs exhibit dramatic performance fluctuation when disturbing the order of the incorporated constraints. Yet, none of the existing works has systematically investigated this position bias problem in the field of multi-constraint instruction following. To bridge this gap, we design a probing task where we quantitatively measure the difficulty distribution of the constraints by a novel Difficulty Distribution Index (CDDI). Through the experimental results, we find that LLMs are more performant when presented with the constraints in a ``hard-to-easy'' order. This preference can be generalized to LLMs with different architecture or different sizes of parameters. Additionally, we conduct an explanation study, providing an intuitive insight into the correlation between the LLM's attention and constraint orders. Our code and dataset are publicly available at https://github.com/meowpass/PBIF.

==> Tab11.tex <==
\begin{table*}[t]
% \resizebox{0.95\textwidth}{!}{
\small
    \begin{tabularx}{\linewidth}{X}
    \toprule
    \color{gray}{/* \textit{Task prompt} */}\\
    You are provided with an <instruction>. Your object is to come up some keywords that may be used to answer the <instruction>. They are usually related to the task described in the <instruction>. you should output your thinking process and the keywords you come up with. \\
    \color{gray}{/* \textit{Example} */}\\
    ---INPUT--- \\
    <instruction>:\\
    Explain Generative Adversarial Networks (GANs) to me using bullet points. Do not contain any commas in your response. \\
    ---OUTPUT---\\
    Thinking process:\\
    The <instruction> asks to explain GANs, hence, 'architecture', 'training' and 'generator' may be appropriate keywords to use in the answer.\\
    Keywords:\\
    \textnormal{[}\texttt{'}architecture\texttt{'}, \texttt{'}training\texttt{'}, \texttt{'}generator\texttt{'}\textnormal{]} \\
    \color{gray}{/* \textit{Input} */}\\
    ---INPUT---\\
    <instruction>:\\
    \{\textbf{Given\_instruction}\}\\
    ---OUTPUT--- \\
    \bottomrule
    \end{tabularx}
    % }
  \caption{
    The prompts for brainstorming some related keywords of a given instruction. The information that requires manual input is highlighted.
  }
  \label{tab:100keyword}
\end{table*}



==> main_res_7cons_all.tex <==
\begin{table*}[t]
\newcolumntype{g}{>{\columncolor{green!10}}c}
%\setlength\tabcolsep{7pt}
\newcolumntype{b}{>{\columncolor{blue!10}}c}

\renewcommand{\arraystretch}{1.22} % 增加行间距到1.5倍
% 在表格环境之前设置全局字体为罗马字体
\renewcommand{\familydefault}{\rmdefault}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccccc}
\toprule
\multirow{2}{*}{Models} & \multirow{2}{*}{BaseModel} &\multicolumn{12}{c}{CDDI} \\
\cmidrule(lr){3-14}
& & \textbf{-1} & \textbf{-0.8} & \textbf{-0.6} & \textbf{-0.4} & \textbf{-0.2} & \textbf{-0.05} & \textbf{0.05} & \textbf{0.2} & \textbf{0.4} & \textbf{0.6} & \textbf{0.8} & \textbf{1}  \\
\midrule
LLaMA2-13B-Chat     & LLaMA2  & 35.79 & 35.82 & 35.99 & 36.09 & 36.01 & 36.59 & 37.06 & 37.28 & 37.89 & 38.36 & 38.49 & 40.09 \\
Mistral-7B-v0.3     & Mistral & 49.59 & 49.75 & 50.06 & 49.69 & 50.23 & 50.04 & 50.39 & 50.47 & 50.30 & 50.79 & 50.63 & 50.68 \\
LLaMA3-8B-Instruct  & LLaMA3  & 53.30 & 53.60 & 53.56 & 55.05 & 55.74 & 56.91 & 56.57 & 57.55 & 59.14 & 60.12 & 60.16 & 60.95 \\
LLaMA3-70B-Instruct & LLaMA3  & 60.15 & 59.85 & 60.81 & 60.69 & 60.84 & 60.79 & 61.11 & 61.56 & 61.64 & 61.31 & 60.99 & 60.16 \\
Qwen2.5-7B-Chat     & Qwen    & 58.25 & 58.46 & 58.69 & 58.56 & 60.40 & 60.35 & 61.34 & 62.35 & 63.27 & 63.24 & 63.36 & 62.76 \\
\bottomrule
\end{tabular}
}
  \caption{
  In single-round inference, the overall performance of LLaMA3-8B-Instruct on multi-constraint instructions with different CDDI.
  }
  \label{tab:main_7cons_all}
\end{table*}


==> main_res_multi_7cons.tex <==
\begin{table*}[t]
\newcolumntype{g}{>{\columncolor{green!10}}c}
%\setlength\tabcolsep{7pt}

\newcolumntype{b}{>{\columncolor{blue!10}}c}
\renewcommand{\arraystretch}{1.22} % 增加行间距到1.5倍
% 在表格环境之前设置全局字体为罗马字体
\renewcommand{\familydefault}{\rmdefault}
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccbg}
\toprule
\textbf{CDDI} & \textbf{Length} & \textbf{keywords} & \textbf{language} & \textbf{ChangeCase} & \textbf{Format} & \textbf{Content} & \textbf{Startend} & \textbf{Punctuation} & \textbf{C\_level} & \textbf{I\_level} \\ \midrule
\textbf{-1}  & \textbf{62.60} & 57.79  & 64.00 & 62.50 & 21.59 & 16.61 & 10.83 & 54.20 & 44.47 & 0.75  \\ 
\textbf{-0.8} & \underline{59.63} & 62.46  & 64.90 & 61.93 & 22.27 & 17.39 & 13.17 & 61.50 & 45.57 & 0.75  \\ 
\textbf{-0.6} & 54.65 & 67.83  & 67.87 & 59.47 & 25.74 & 20.08 & 22.75 & 65.67 & 47.40 & 0.65  \\ 
\textbf{-0.4} & 52.77 & 69.57  & 68.74 & 61.44 & 32.30 & 26.21 & 30.78 & 64.46 & 49.98 & 1.05  \\ 
\textbf{-0.2} & 48.73 & 74.67  & 68.74 & 59.16 & 38.67 & 32.02 & 39.00 & 62.42 & 52.07 & 1.25  \\ 
\textbf{-0.05} & 46.48 & 76.04 & 69.97 & 60.97 & 46.38 & 46.58 & 48.79 & 67.17 & 56.35 & 1.40  \\ \cdashlinelr{1-11} 
\textbf{0.05}  & 45.32 & 76.62 & 70.08 & 62.18 & 51.19 & 50.47 & 52.68 & 68.84 & 58.04 & 1.80  \\ 
\textbf{0.2}   & 44.81 & 80.20 & 69.91 & 60.34 & 58.35 & 63.22 & 62.41 & 66.73 & 61.79 & 3.41  \\ 
\textbf{0.4}   & 44.30 & 81.75 & \textbf{72.50} & \underline{63.50} & 64.50 & 73.56 & 68.00 & \underline{69.10} & 65.39 & \underline{5.60}  \\ 
\textbf{0.6}   & 43.71 & 83.87 & 68.87 & 59.83 & 71.71 & 81.77 & 71.98 & 68.20 & 67.47 & 5.05  \\ 
\textbf{0.8}   & 44.35 & \underline{84}.49 & 68.37 & 61.54 & \underline{75.94} & \underline{84.88} & \underline{70.31} & 68.00 & \underline{68.76} & \textbf{6.00}  \\ 
\textbf{1}     & 44.07 &\textbf{85.08} & \underline{70.90} & \textbf{64.43} & \textbf{81.41} & \textbf{87.22} & \textbf{72.58} & \textbf{69.60} & \textbf{70.74} & 4.00  \\ \bottomrule
\end{tabular}
}
  \caption{
    In multi-round inference, the overall performance of LLaMA3-8B-Instruct on multi-constraint instructions with different CDDI
  }
  \label{tab:main_multi_7cons}
\end{table*}

